Breaking the Sorting Barrier for Directed Single-Source Shortest Paths

We give a deterministic $O(m\log^{2/3}n)$-time algorithm for single-source shortest paths (SSSP) on directed graphs with real non-negative edge weights in the comparison-addition model. This is the first result to break the $O(m+n\log n)$ time bound of Dijkstra's algorithm on sparse graphs, showing that Dijkstra's algorithm is not optimal for SSSP.

==> discussion.tex <==
\section{Discussion}\label{sec:discussion}
%\xiao{maybe rename this to more accurately state that we are talking about that popular lower-bound result?}

Although our algorithm constructs a hierarchy on subsets of vertices, it still breaks the lower bound for ``hierarchy-based'' algorithms in~\cite{PR05}. This is because our algorithm does not satisfy the ``hierarchy property'' (Property 6.1 in~\cite{PR05}), which mainly comes from \textsc{FindPivots} procedure which deals with shortest paths of a small number of edges. In the counterexample of Theorem 6.1 in~\cite{PR05}, \textsc{FindPivots} procedure can find all the distances without sorting them.
